Occ-VLM: Occupancy Grounded Vision Language Model for Indoor Scene Understanding

Recently, vision-language models (VLMs) have made significant progress in 3D scene understanding, driving advances in applications such as embodied intelligence and robotic vision. However, existing approaches typically either rely directly on explicit 3D inputs (e.g., point clouds or RGB-D sequences), or introduce an additional 3D geometry encoder to derive 3D-aware visual tokens from 2D images. Such designs structurally decouple 3D geometric perception from the rich 2D semantics learned via vision-language pre-training, hindering the development of a unified 3D vision-language representation. In this work, we propose Occ-VLM, a novel framework for 3D scene understanding that operates purely on posed RGB images and employs a single 2D vision encoder. Specifically, Occ-VLM reconstructs 3D scene occupancy as an auxiliary geometric prior, which is utilized to spatially associate foreground 2D tokens with 3D space. These tokens are then decoded by a Large Language Model (LLM) for unified scene understanding. Extensive experiments demonstrate that Occ-VLM achieves both accurate geometric perception and robust vision-language reasoning: it attains state-of-the-art performance on multi-view occupancy prediction, while performing on par with 3D-input VLMs on 3D Visual Question Answering (VQA) and 3D dense captioning benchmarks.

==> sec/0_abstract.tex <==
\begin{abstract}



\end{abstract}


% 近年来，大规模视觉语言模型（LVLMs）的视觉Token压缩取得了显著进展，其目标是在保留性能的同时减少计算冗余，主要依赖于二维领域的语义驱动Token剪枝。然而，当这一类方法应用于三维视觉Token时，面临着根本性限制——由于三维Token具有复杂的空间几何分布，仅依靠语义重要性指标难以捕捉关键的结构关系。为此，我们提出了SGViCo，一种基于几何信息的压缩框架，通过两个互补阶段对三维视觉Token进行分层优化：1）语义Token剪枝：在三维投影之前，先剔除低信息量的二维图像Token；2）几何Token合并：基于几何分布对三维Token进行聚类，并采用空间感知的合并策略，进一步减少Token数量，同时保留关键的三维结构线索。在三维视觉问答基准测试上的大量实验结果表明，SGViCo在实现50% Token压缩的同时，准确率下降小于5.0%，不仅优于二维压缩方法的基线效果，还保持了最先进的任务性能。



%难以有效捕捉三维空间关系与语义信息，导致其在三维视觉语言任务(如三维视觉问答)中性能受限。为此，我们提出一种创新的三维视觉令牌压缩框架SGViCo，
